META-CAT: Speaker-Informed Speech Embeddings via Meta Information Concatenation for Multi-talker ASR

We propose a novel end-to-end multi-talker automatic speech recognition (ASR) framework that enables both multi-speaker (MS) ASR and target-speaker (TS) ASR. Our proposed model is trained in a fully end-to-end manner, incorporating speaker supervision from a pre-trained speaker diarization module. We introduce an intuitive yet effective method for masking ASR encoder activations using output from the speaker supervision module, a technique we term Meta-Cat (meta-information concatenation), that can be applied to both MS-ASR and TS-ASR. Our results demonstrate that the proposed architecture achieves competitive performance in both MS-ASR and TS-ASR tasks, without the need for traditional methods, such as neural mask estimation or masking at the audio or feature level. Furthermore, we demonstrate a glimpse of a unified dual-task model which can efficiently handle both MS-ASR and TS-ASR tasks. Thus, this work illustrates that a robust end-to-end multi-talker ASR framework can be implemented with a streamlined architecture, obviating the need for the complex speaker filtering mechanisms employed in previous studies.

==> Chapters/Chapter_1B.tex <==
\section{Related Work}

\textbf{Speaker diarization and ASR}: Before the widespread adoption of multi-speaker automatic speech recognition (ASR), the task of determining "who spoke when" was primarily addressed through speaker diarization. Speaker diarization assigns speaker labels to specific audio frames without transcribing the speech. Though distinct tasks, many studies have explored integrating speaker diarization and ASR.

Early efforts, such as during the RT03 evaluation~\cite{tranter2003investigation}, used ASR output for speaker diarization, utilizing word boundary information for segmentation. While the improvement was modest, it marked the first attempt to enhance diarization using ASR-based segmentation. Later systems, like those in~\cite{huang2007ibm} and~\cite{silovsky2012incorporation}, improved speaker activity detection and addressed word breakage issues. Canseco et al.~\cite{canseco2004speaker} further advanced this integration by developing a dictionary of common phrases to aid speaker identification.
Recent approaches have leveraged neural models to incorporate ASR output for better performance. Flemotomos et al.\cite{flemotomos2019linguistically} reduced the diarization error rate (DER) by combining linguistic and acoustic information using a neural text-based speaker change detector. Park et al.\cite{park2018multimodal, park2019speaker} also demonstrated that combining lexical and acoustic data improves diarization accuracy.
In modular, pipelined multi-speaker ASR, the CHiME Challenges~\cite{vincent20164th, watanabe2020chime, cornell2023chime} have significantly advanced the field. Medennikov et al.\cite{medennikov2020stc} proposed a prominent multi-speaker ASR system for the CHiME-6 Challenge~\cite{watanabe2020chime}, using a target-speaker voice activity detector (TS-VAD) to accurately transcribe multi-speaker audio mixtures.

\textbf{End-to-end Multi-Speaker ASR}: \cite{qian2018single} demonstrated that an end-to-end multi-speaker ASR system could be created using multiple single-speaker ASR modules. \cite{yu17b_interspeech} extended this idea by recognizing two speakers with a single ASR model using permutation-free training with RNN-T-based modules. \cite{seki2018end} combined source separation with speech recognition, using a CTC-based loss, while ~\cite{shafey2019joint} introduced a jointly trainable RNN-T model for simultaneous speaker label and text token generation. \cite{chang2019end} added an attention mechanism for training a multi-speaker ASR model without alignments or non-mixture labels, which was later expanded into the Multi-channel Input Multiple Output (MIMO) system~\cite{chang2019mimo}.

A major advancement came with ~\cite{kanda2020serialized}'s Serialized Output Training (SOT) method, which simplified end-to-end multi-speaker ASR by utilizing the Transformer architecture's multi-head attention, eliminating the need for neural mask estimators. This system processes overlapping speech using attention values, relying solely on multi-head self-attention. SOT was later extended to a token-level version (t-SOT) for streaming systems~\cite{kanda2022streaming}. Recently, \cite{cornell2024one} introduced a joint system for speaker diarization and speech recognition, handling multi-speaker ASR with speaker clustering later in the process.
 
\textbf{End-to-end Target-Speaker ASR}: Target-speaker automatic speech recognition (TS-ASR) is an advanced method developed to transcribe the speech of a specific speaker in environments where multiple speakers are talking simultaneously. In contrast to blind source separation (BSS) \cite{luo2019conv,subakan2021attention} and multi-speaker ASR, which attempt to separate or recognize all speakers in a given audio mixture, TS-ASR focuses exclusively on the target speaker by using an auxiliary utterance—essentially a clean sample of the target speaker’s voice. This allows TS-ASR to transcribe the desired speaker’s speech while disregarding other interfering voices in the background \cite{delcroix2018single, vzmolikova2019speakerbeam, moriya2022streaming, kanda19_interspeech}. The approach has become crucial for various applications, such as voice assistants, personal communication devices, and meeting transcription systems, where capturing a specific speaker’s speech accurately is of paramount importance.


